Model-Based Development of Distributed Embedded Systems by the Example of the Scicos/SynDEx Framework

The embedded systems engineering industry faces increasing demands for more functionality, rapidly evolving components, and shrinking schedules. Abilities to quickly adapt to changes, develop products with safe design, minimize project costs, and deliver timely are needed. Model-based development (MBD) follows a separation of concerns by abstracting systems with an appropriate intensity. MBD promises higher comprehension by modeling on several abstraction-levels, formal verification, and automated code generation. This thesis demonstrates MBD with the Scicos/SynDEx framework on a distributed embedded system. Scicos is a modeling and simulation environment for hybrid systems. SynDEx is a rapid prototyping integrated development environment for distributed systems. Performed examples implement well-known control algorithms on a target system containing several networked microcontrollers, sensors, and actuators. The addressed research question tackles the feasibility of MBD for medium-sized embedded systems. In the case of single-processor applications experiments show that the comforts of tool-provided simulation, verification, and code-generation have to be weighed against an additional memory consumption in dynamic and static memory compared to a hand-written approach. Establishing a near-seamless modeling-framework with Scicos/SynDEx is expensive. An increased development effort indicates a high price for developing single applications, but might pay off for product families. A further drawback was that the distributed code generated with SynDEx could not be adapted to microcontrollers without a significant alteration of the scheduling tables. The Scicos/SynDEx framework forms a valuable tool set that, however, still needs many improvements. Therefore, its usage is only recommended for experimental purposes.

==> a/titlepage.tex <==
\title{Model-Based Development of Distributed Embedded Systems by the Example of the Scicos/SynDEx Framework}
\author{Bernhard Fischer}
\address{Dr. Karl Rennerring 31, A-8940 Liezen}
\matrikel{0126057}
\date{09 2010}

\renewcommand{\dankname}{}
